ASPIC: Proof-of-Concept ASP to Picat Transpiler

This article presents ASPIC, a new proof-of-concept library that converts extended syntax ASP-Core-2 programs to Picat predicates that can be solved right away with the integrated Picat SAT solver, or embedded in larger Picat programs ("ASP in Picat"), and that can in turn make use of various Picat predicates and functions ("Picat in ASP"). The first tests prove good compatibility with clingo, on programs lacking positive loops and when the special Picat features are not used. With the embedded Picat, it touches the application field of clingcon as well, by being able to efficiently model with both ASP atoms and with finite domain variables, but goes beyond that by being able to model also non-linear constraints.

==> eptcsdata.tex <==
\providecommand{\firstpage}{270}
\providecommand{\publicationstatus}{W. Faber, L. Giordano, R. Rocha, V. Santos Costa (Eds.):\\ 42nd International Conference on Logic Programming (ICLP 2026)\\
EPTCS 450, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.450.21}{10.4204/EPTCS.450.21}}

